Measurement of the time-integrated $CP$ asymmetry in $D^0\to\pi^0\pi^0$ decays at Belle II

We measure the time-integrated $CP$ asymmetry, $A_{CP}$, in $D^0\to\pi^0\pi^0$ decays reconstructed in $e^+e^-\to c\bar{c}$ events collected by Belle II during 2019--2022. The data corresponds to an integrated luminosity of 428$\mathrm{fb}^{-1}$. The $D^0$ decays are required to originate from the flavor-conserving $D^{*+} \to D^0 \pi^+$ decay to determine the charm flavor at production time. Control samples of $D^0\to K^- \pi^+$ decays, with or without an associated pion from a $D^{*+}$ decay, are used to correct for detection asymmetries. The result, $A_{CP}(D^0\to\pi^0\pi^0) = (0.30\pm 0.72\pm 0.20)\%$, where the first uncertainty is statistical and the second systematic, is consistent with $CP$ symmetry.

==> authors/pub080-orcid.tex <==
%%% Paper:    D0 to pi0 pi0
%%% Journal:  PhysRev
%%% Contacts: M. Bertemes, A. Di Canto
%%% ====================================================================
%%% Use \input{pub080-orcid} to insert this material into your latex file.
  \author{I.~Adachi\,\orcidlink{0000-0003-2287-0173}} % 2590
% \author{K.~Adamczyk\,\orcidlink{0000-0001-6208-0876}} % 2239
% \author{L.~Aggarwal\,\orcidlink{0000-0002-0909-7537}} % 10083
% \author{P.~Ahlburg\,\orcidlink{0000-0002-9832-7604}} % 2367
% \author{H.~Ahmed\,\orcidlink{0000-0003-3976-7498}} % 11323
% \author{J.~K.~Ahn\,\orcidlink{0000-0002-5795-2243}} % 7423
  \author{Y.~Ahn\,\orcidlink{0000-0001-6820-0576}} % 14363
% \author{H.~Aihara\,\orcidlink{0000-0002-1907-5964}} % 2223
  \author{N.~Akopov\,\orcidlink{0000-0002-4425-2096}} % 9443
  \author{S.~Alghamdi\,\orcidlink{0000-0001-7609-112X}} % 27804
  \author{M.~Alhakami\,\orcidlink{0000-0002-2234-8628}} % 28103
  \author{A.~Aloisio\,\orcidlink{0000-0002-3883-6693}} % 2194
  \author{N.~Althubiti\,\orcidlink{0000-0003-1513-0409}} % 21524
  \author{K.~Amos\,\orcidlink{0000-0003-1757-5620}} % 27583
% \author{L.~Andricek\,\orcidlink{0000-0003-1755-4475}} % 2098
  \author{M.~Angelsmark\,\orcidlink{0000-0003-4745-1020}} % 13963
  \author{N.~Anh~Ky\,\orcidlink{0000-0003-0471-197X}} % 2218
  \author{C.~Antonioli\,\orcidlink{0009-0003-9088-3811}} % 20583
  \author{D.~M.~Asner\,\orcidlink{0000-0002-1586-5790}} % 4684
  \author{H.~Atmacan\,\orcidlink{0000-0003-2435-501X}} % 2538
% \author{V.~Aulchenko\,\orcidlink{0000-0002-5394-4406}} % 8183
  \author{T.~Aushev\,\orcidlink{0000-0002-6347-7055}} % 3747
% \author{V.~Aushev\,\orcidlink{0000-0002-8588-5308}} % 2155
  \author{M.~Aversano\,\orcidlink{0000-0001-9980-0953}} % 7363
  \author{R.~Ayad\,\orcidlink{0000-0003-3466-9290}} % 3766
% \author{T.~Aziz\,\orcidlink{-}} % 3523
  \author{V.~Babu\,\orcidlink{0000-0003-0419-6912}} % 5623
% \author{S.~Bacher\,\orcidlink{0000-0002-2656-2330}} % 2258
  \author{H.~Bae\,\orcidlink{0000-0003-1393-8631}} % 10863
  \author{N.~K.~Baghel\,\orcidlink{0009-0008-7806-4422}} % 21505
  \author{S.~Bahinipati\,\orcidlink{0000-0002-3744-5332}} % 2332
% \author{A.~M.~Bakich\,\orcidlink{0000-0001-8315-4854}} % 2115
  \author{P.~Bambade\,\orcidlink{0000-0001-7378-4852}} % 3003
  \author{Sw.~Banerjee\,\orcidlink{0000-0001-8852-2409}} % 8603
% \author{S.~Bansal\,\orcidlink{0000-0003-1992-0336}} % 5163
  \author{M.~Barrett\,\orcidlink{0000-0002-2095-603X}} % 2180
  \author{M.~Bartl\,\orcidlink{0009-0002-7835-0855}} % 26483
% \author{G.~Batignani\,\orcidlink{0000-0003-3917-3104}} % 6643
  \author{J.~Baudot\,\orcidlink{0000-0001-5585-0991}} % 2562
% \author{M.~Bauer\,\orcidlink{0000-0002-0953-7387}} % 9863
  \author{A.~Baur\,\orcidlink{0000-0003-1360-3292}} % 5683
  \author{A.~Beaubien\,\orcidlink{0000-0001-9438-089X}} % 6683
  \author{F.~Becherer\,\orcidlink{0000-0003-0562-4616}} % 21623
  \author{J.~Becker\,\orcidlink{0000-0002-5082-5487}} % 5403
% \author{P.~K.~Behera\,\orcidlink{0000-0002-1527-2266}} % 4204
  \author{J.~V.~Bennett\,\orcidlink{0000-0002-5440-2668}} % 2454
% \author{E.~Bernieri\,\orcidlink{0000-0002-4787-2047}} % 4483
  \author{F.~U.~Bernlochner\,\orcidlink{0000-0001-8153-2719}} % 2282
  \author{V.~Bertacchi\,\orcidlink{0000-0001-9971-1176}} % 2212
  \author{M.~Bertemes\,\orcidlink{0000-0001-5038-360X}} % 2595
  \author{E.~Bertholet\,\orcidlink{0000-0002-3792-2450}} % 13163
  \author{M.~Bessner\,\orcidlink{0000-0003-1776-0439}} % 3783
% \author{D.~Z.~Besson\,\orcidlink{-}} % 3585
  \author{S.~Bettarini\,\orcidlink{0000-0001-7742-2998}} % 2350
% \author{V.~Bhardwaj\,\orcidlink{0000-0001-8857-8621}} % 2228
  \author{B.~Bhuyan\,\orcidlink{0000-0001-6254-3594}} % 2097
  \author{F.~Bianchi\,\orcidlink{0000-0002-1524-6236}} % 2564
% \author{L.~Bierwirth\,\orcidlink{0009-0003-0192-9073}} % 11723
  \author{T.~Bilka\,\orcidlink{0000-0003-1449-6986}} % 2484
% \author{S.~Bilokin\,\orcidlink{0000-0003-0017-6260}} % 3623
  \author{D.~Biswas\,\orcidlink{0000-0002-7543-3471}} % 8703
% \author{T.~Bloomfield\,\orcidlink{0000-0001-9288-5069}} % 2418
  \author{A.~Bobrov\,\orcidlink{0000-0001-5735-8386}} % 2294
  \author{D.~Bodrov\,\orcidlink{0000-0001-5279-4787}} % 9643
% \author{A.~Bolz\,\orcidlink{0000-0002-4033-9223}} % 15403
  \author{A.~Bondar\,\orcidlink{0000-0002-5089-5338}} % 4643
% \author{G.~Bonvicini\,\orcidlink{0000-0003-4861-7918}} % 2095
  \author{J.~Borah\,\orcidlink{0000-0003-2990-1913}} % 7083
  \author{A.~Boschetti\,\orcidlink{0000-0001-6030-3087}} % 17683
  \author{A.~Bozek\,\orcidlink{0000-0002-5915-1319}} % 2303
  \author{M.~Bra\v{c}ko\,\orcidlink{0000-0002-2495-0524}} % 2425
  \author{P.~Branchini\,\orcidlink{0000-0002-2270-9673}} % 2577
% \author{N.~Brenny\,\orcidlink{0009-0006-2917-9173}} % 19943
  \author{R.~A.~Briere\,\orcidlink{0000-0001-5229-1039}} % 2584
  \author{T.~E.~Browder\,\orcidlink{0000-0001-7357-9007}} % 2560
% \author{Y.~Buch\,\orcidlink{0000-0002-8050-4000}} % 17323
  \author{A.~Budano\,\orcidlink{0000-0002-0856-1131}} % 2171
  \author{S.~Bussino\,\orcidlink{0000-0002-3829-9592}} % 5384
% \author{A.~Calcaterra\,\orcidlink{0000-0003-2670-4826}} % 19163
% \author{A.~Caldwell\,\orcidlink{-}} % 2608
% \author{Q.~Campagna\,\orcidlink{0000-0002-3109-2046}} % 21563
  \author{M.~Campajola\,\orcidlink{0000-0003-2518-7134}} % 5223
  \author{L.~Cao\,\orcidlink{0000-0001-8332-5668}} % 2099
  \author{G.~Casarosa\,\orcidlink{0000-0003-4137-938X}} % 2491
  \author{C.~Cecchi\,\orcidlink{0000-0002-2192-8233}} % 2433
% \author{J.~Cerasoli\,\orcidlink{0000-0001-9777-881X}} % 20746
% \author{M.-C.~Chang\,\orcidlink{0000-0002-8650-6058}} % 2827
% \author{P.~Chang\,\orcidlink{0000-0003-4064-388X}} % 2542
% \author{R.~Cheaib\,\orcidlink{0000-0001-5729-8926}} % 2208
  \author{P.~Cheema\,\orcidlink{0000-0001-8472-5727}} % 15264
% \author{V.~Chekelian\,\orcidlink{0000-0001-8860-8288}} % 2167
% \author{C.~Chen\,\orcidlink{0000-0003-1589-9955}} % 12803
% \author{Y.-T.~Chen\,\orcidlink{0000-0003-2639-2850}} % 2884
  \author{B.~G.~Cheon\,\orcidlink{0000-0002-8803-4429}} % 2173
  \author{K.~Chilikin\,\orcidlink{0000-0001-7620-2053}} % 2308
  \author{J.~Chin\,\orcidlink{0009-0005-9210-8872}} % 20283
  \author{K.~Chirapatpimol\,\orcidlink{0000-0003-2099-7760}} % 10803
  \author{H.-E.~Cho\,\orcidlink{0000-0002-7008-3759}} % 2182
  \author{K.~Cho\,\orcidlink{0000-0003-1705-7399}} % 2516
  \author{S.-J.~Cho\,\orcidlink{0000-0002-1673-5664}} % 2723
  \author{S.-K.~Choi\,\orcidlink{0000-0003-2747-8277}} % 2364
  \author{S.~Choudhury\,\orcidlink{0000-0001-9841-0216}} % 2206
% \author{K.~Chu\,\orcidlink{0000-0002-1997-4249}} % 5203
% \author{D.~Cinabro\,\orcidlink{0000-0001-7347-6585}} % 2092
% \author{J.~Cochran\,\orcidlink{0000-0002-1492-914X}} % 12604
  \author{I.~Consigny\,\orcidlink{0009-0009-8755-6290}} % 23903
  \author{L.~Corona\,\orcidlink{0000-0002-2577-9909}} % 3944
% \author{L.~M.~Cremaldi\,\orcidlink{0000-0001-5550-7827}} % 2276
  \author{J.~X.~Cui\,\orcidlink{0000-0002-2398-3754}} % 8863
% \author{T.~Czank\,\orcidlink{0000-0001-6621-3373}} % 2254
% \author{S.~Das\,\orcidlink{0000-0001-6857-966X}} % 9163
% \author{F.~Dattola\,\orcidlink{0000-0003-3316-8574}} % 3745
  \author{E.~De~La~Cruz-Burelo\,\orcidlink{0000-0002-7469-6974}} % 2359
  \author{S.~A.~De~La~Motte\,\orcidlink{0000-0003-3905-6805}} % 2128
% \author{G.~de~Marino\,\orcidlink{0000-0002-6509-7793}} % 8364
% \author{G.~De~Nardo\,\orcidlink{0000-0002-2047-9675}} % 2459
% \author{M.~De~Nuccio\,\orcidlink{0000-0002-0972-9047}} % 2610
  \author{G.~De~Pietro\,\orcidlink{0000-0001-8442-107X}} % 2528
  \author{R.~de~Sangro\,\orcidlink{0000-0002-3808-5455}} % 2524
% \author{B.~Deschamps\,\orcidlink{0000-0003-2497-5008}} % 2671
  \author{M.~Destefanis\,\orcidlink{0000-0003-1997-6751}} % 2594
% \author{S.~Dey\,\orcidlink{0000-0003-2997-3829}} % 5023
% \author{A.~De~Yta-Hernandez\,\orcidlink{0000-0002-2162-7334}} % 2104
% \author{R.~Dhamija\,\orcidlink{0000-0001-7052-3163}} % 9465
  \author{A.~Di~Canto\,\orcidlink{0000-0003-1233-3876}} % 10963
% \author{F.~Di~Capua\,\orcidlink{0000-0001-9076-5936}} % 2065
  \author{J.~Dingfelder\,\orcidlink{0000-0001-5767-2121}} % 2151
  \author{Z.~Dole\v{z}al\,\orcidlink{0000-0002-5662-3675}} % 2319
  \author{I.~Dom\'{\i}nguez~Jim\'{e}nez\,\orcidlink{0000-0001-6831-3159}} % 2191
  \author{T.~V.~Dong\,\orcidlink{0000-0003-3043-1939}} % 2215
% \author{X.~Dong\,\orcidlink{0000-0001-8574-9624}} % 17343
  \author{M.~Dorigo\,\orcidlink{0000-0002-0681-6946}} % 12543
% \author{D.~Dorner\,\orcidlink{0000-0003-3628-9267}} % 13564
% \author{K.~Dort\,\orcidlink{0000-0003-0849-8774}} % 5583
% \author{D.~Dossett\,\orcidlink{0000-0002-5670-5582}} % 2574
% \author{S.~Dreyer\,\orcidlink{0000-0002-6295-100X}} % 12823
% \author{S.~Dubey\,\orcidlink{0000-0002-1345-0970}} % 11063
% \author{S.~Duell\,\orcidlink{0000-0001-9918-9808}} % 2344
% \author{K.~Dugic\,\orcidlink{0009-0006-6056-546X}} % 11103
  \author{G.~Dujany\,\orcidlink{0000-0002-1345-8163}} % 9703
  \author{P.~Ecker\,\orcidlink{0000-0002-6817-6868}} % 5563
% \author{M.~Eliachevitch\,\orcidlink{0000-0003-2033-537X}} % 2725
  \author{D.~Epifanov\,\orcidlink{0000-0001-8656-2693}} % 2551
  \author{J.~Eppelt\,\orcidlink{0000-0001-8368-3721}} % 19723
% \author{Y.~Fan\,\orcidlink{0000-0001-9616-9705}} % 21303
  \author{R.~Farkas\,\orcidlink{0000-0002-7647-1429}} % 12843
  \author{P.~Feichtinger\,\orcidlink{0000-0003-3966-7497}} % 9843
  \author{T.~Ferber\,\orcidlink{0000-0002-6849-0427}} % 2482
% \author{D.~Ferlewicz\,\orcidlink{0000-0002-4374-1234}} % 2073
  \author{T.~Fillinger\,\orcidlink{0000-0001-9795-7412}} % 9803
  \author{C.~Finck\,\orcidlink{0000-0002-5068-5453}} % 15803
  \author{G.~Finocchiaro\,\orcidlink{0000-0002-3936-2151}} % 2400
% \author{P.~Fischer\,\orcidlink{0000-0002-9808-3574}} % 2141
% \author{K.~Flood\,\orcidlink{0000-0002-3463-6571}} % 12103
  \author{A.~Fodor\,\orcidlink{0000-0002-2821-759X}} % 2312
  \author{F.~Forti\,\orcidlink{0000-0001-6535-7965}} % 2432
% \author{A.~Frey\,\orcidlink{0000-0001-7470-3874}} % 2150
% \author{M.~Friedl\,\orcidlink{0000-0002-7420-2559}} % 2442
  \author{B.~G.~Fulsom\,\orcidlink{0000-0002-5862-9739}} % 2563
  \author{A.~Gabrielli\,\orcidlink{0000-0001-7695-0537}} % 13523
% \author{N.~Gabyshev\,\orcidlink{0000-0002-8593-6857}} % 2510
  \author{A.~Gale\,\orcidlink{0009-0005-2634-7189}} % 20263
  \author{E.~Ganiev\,\orcidlink{0000-0001-8346-8597}} % 4623
  \author{M.~Garcia-Hernandez\,\orcidlink{0000-0003-2393-3367}} % 4823
  \author{R.~Garg\,\orcidlink{0000-0002-7406-4707}} % 2213
% \author{A.~Garmash\,\orcidlink{0000-0003-2599-1405}} % 2161
% \author{L.~G\"artner\,\orcidlink{0000-0002-3643-4543}} % 21783
  \author{G.~Gaudino\,\orcidlink{0000-0001-5983-1552}} % 16563
  \author{V.~Gaur\,\orcidlink{0000-0002-8880-6134}} % 2413
  \author{V.~Gautam\,\orcidlink{0009-0001-9817-8637}} % 22223
  \author{A.~Gaz\,\orcidlink{0000-0001-6754-3315}} % 2181
  \author{A.~Gellrich\,\orcidlink{0000-0003-0974-6231}} % 2480
% \author{G.~Ghevondyan\,\orcidlink{0000-0003-0096-3555}} % 9445
  \author{D.~Ghosh\,\orcidlink{0000-0002-3458-9824}} % 11923
  \author{H.~Ghumaryan\,\orcidlink{0000-0001-6775-8893}} % 19543
  \author{G.~Giakoustidis\,\orcidlink{0000-0001-5982-1784}} % 13723
  \author{R.~Giordano\,\orcidlink{0000-0002-5496-7247}} % 2103
  \author{A.~Giri\,\orcidlink{0000-0002-8895-0128}} % 2106
  \author{P.~Gironella~Gironell\,\orcidlink{0000-0001-5603-4750}} % 25443
% \author{A.~Glazov\,\orcidlink{0000-0002-8553-7338}} % 2473
  \author{B.~Gobbo\,\orcidlink{0000-0002-3147-4562}} % 2109
  \author{R.~Godang\,\orcidlink{0000-0002-8317-0579}} % 2449
  \author{O.~Gogota\,\orcidlink{0000-0003-4108-7256}} % 2334
  \author{P.~Goldenzweig\,\orcidlink{0000-0001-8785-847X}} % 2345
% \author{B.~Golob\,\orcidlink{0000-0001-9632-5616}} % 3703
% \author{G.~Gong\,\orcidlink{0000-0001-7192-1833}} % 2727
% \author{P.~Grace\,\orcidlink{0000-0001-9005-7403}} % 9563
  \author{W.~Gradl\,\orcidlink{0000-0002-9974-8320}} % 2570
% \author{M.~Graf-Schreiber\,\orcidlink{0000-0003-4613-1041}} % 2730
% \author{T.~Grammatico\,\orcidlink{0000-0002-2818-9744}} % 20623
% \author{S.~Granderath\,\orcidlink{0000-0002-9945-463X}} % 8383
  \author{E.~Graziani\,\orcidlink{0000-0001-8602-5652}} % 2342
  \author{D.~Greenwald\,\orcidlink{0000-0001-6964-8399}} % 2686
  \author{Z.~Gruberov\'{a}\,\orcidlink{0000-0002-5691-1044}} % 8824
% \author{T.~Gu\,\orcidlink{0000-0002-1470-6536}} % 14283
% \author{Y.~Guan\,\orcidlink{0000-0002-5541-2278}} % 2514
  \author{K.~Gudkova\,\orcidlink{0000-0002-5858-3187}} % 10504
  \author{I.~Haide\,\orcidlink{0000-0003-0962-6344}} % 14824
% \author{H.~Haigh\,\orcidlink{0000-0003-1567-0907}} % 16744
% \author{S.~Halder\,\orcidlink{0000-0002-6280-494X}} % 4743
  \author{Y.~Han\,\orcidlink{0000-0001-6775-5932}} % 19663
% \author{K.~Hara\,\orcidlink{0000-0002-5361-1871}} % 2462
% \author{T.~Hara\,\orcidlink{0000-0002-4321-0417}} % 2523
% \author{C.~Harris\,\orcidlink{0000-0003-0448-4244}} % 21383
% \author{K.~Hayasaka\,\orcidlink{0000-0002-6347-433X}} % 2330
  \author{H.~Hayashii\,\orcidlink{0000-0002-5138-5903}} % 2455
  \author{S.~Hazra\,\orcidlink{0000-0001-6954-9593}} % 7663
  \author{C.~Hearty\,\orcidlink{0000-0001-6568-0252}} % 2450
  \author{M.~T.~Hedges\,\orcidlink{0000-0001-6504-1872}} % 2265
  \author{A.~Heidelbach\,\orcidlink{0000-0002-6663-5469}} % 16923
  \author{G.~Heine\,\orcidlink{0009-0009-1827-2008}} % 23863
  \author{I.~Heredia~de~la~Cruz\,\orcidlink{0000-0002-8133-6467}} % 2559
  \author{M.~Hern\'{a}ndez~Villanueva\,\orcidlink{0000-0002-6322-5587}} % 2466
  \author{T.~Higuchi\,\orcidlink{0000-0002-7761-3505}} % 2485
% \author{H.~Hirata\,\orcidlink{0000-0001-9005-4616}} % 2070
  \author{M.~Hoek\,\orcidlink{0000-0002-1893-8764}} % 2101
  \author{M.~Hohmann\,\orcidlink{0000-0001-5147-4781}} % 2077
% \author{R.~Hoppe\,\orcidlink{0009-0005-8881-8935}} % 23383
  \author{P.~Horak\,\orcidlink{0000-0001-9979-6501}} % 13583
% \author{T.~Hotta\,\orcidlink{0000-0002-1079-5826}} % 2084
  \author{C.-L.~Hsu\,\orcidlink{0000-0002-1641-430X}} % 2299
% \author{A.~Huang\,\orcidlink{0000-0003-1748-7348}} % 14223
% \author{K.~Huang\,\orcidlink{0000-0001-9342-7406}} % 2389
% \author{T.~Humair\,\orcidlink{0000-0002-2922-9779}} % 10643
  \author{T.~Iijima\,\orcidlink{0000-0002-4271-711X}} % 2446
  \author{K.~Inami\,\orcidlink{0000-0003-2765-7072}} % 2323
  \author{G.~Inguglia\,\orcidlink{0000-0003-0331-8279}} % 2500
  \author{N.~Ipsita\,\orcidlink{0000-0002-2927-3366}} % 12223
% \author{C.~Irmler\,\orcidlink{-}} % 2186
  \author{A.~Ishikawa\,\orcidlink{0000-0002-3561-5633}} % 2281
  \author{R.~Itoh\,\orcidlink{0000-0003-1590-0266}} % 2487
  \author{M.~Iwasaki\,\orcidlink{0000-0002-9402-7559}} % 2360
% \author{Y.~Iwasaki\,\orcidlink{0000-0001-7261-2557}} % 2229
% \author{S.~Iwata\,\orcidlink{0009-0005-5017-8098}} % 4323
  \author{P.~Jackson\,\orcidlink{0000-0002-0847-402X}} % 2255
  \author{D.~Jacobi\,\orcidlink{0000-0003-2399-9796}} % 15123
  \author{W.~W.~Jacobs\,\orcidlink{0000-0002-9996-6336}} % 2322
  \author{D.~E.~Jaffe\,\orcidlink{0000-0003-3122-4384}} % 3663
% \author{E.-J.~Jang\,\orcidlink{0000-0002-1935-9887}} % 6744
  \author{Q.~P.~Ji\,\orcidlink{0000-0003-2963-2565}} % 16243
% \author{X.~B.~Ji\,\orcidlink{0000-0002-6337-5040}} % 2558
  \author{S.~Jia\,\orcidlink{0000-0001-8176-8545}} % 2457
  \author{Y.~Jin\,\orcidlink{0000-0002-7323-0830}} % 2105
  \author{A.~Johnson\,\orcidlink{0000-0002-8366-1749}} % 16143
% \author{K.~K.~Joo\,\orcidlink{0000-0002-5515-0087}} % 4224
% \author{H.~Junkerkalefeld\,\orcidlink{0000-0003-3987-9895}} % 12963
% \author{I.~Kadenko\,\orcidlink{0000-0001-8766-4229}} % 3843
% \author{H.~Kakuno\,\orcidlink{0000-0002-9957-6055}} % 2391
% \author{M.~Kaleta\,\orcidlink{0000-0002-2863-5476}} % 5603
% \author{D.~Kalita\,\orcidlink{0000-0003-3054-1222}} % 2220
% \author{A.~B.~Kaliyar\,\orcidlink{0000-0002-2211-619X}} % 7344
  \author{J.~Kandra\,\orcidlink{0000-0001-5635-1000}} % 2541
  \author{K.~H.~Kang\,\orcidlink{0000-0002-6816-0751}} % 2283
% \author{S.~Kang\,\orcidlink{0000-0002-5320-7043}} % 12683
  \author{G.~Karyan\,\orcidlink{0000-0001-5365-3716}} % 2550
% \author{H.~Kawai\,\orcidlink{-}} % 4344
  \author{T.~Kawasaki\,\orcidlink{0000-0002-4089-5238}} % 4363
  \author{F.~Keil\,\orcidlink{0000-0002-7278-2860}} % 19523
  \author{C.~Ketter\,\orcidlink{0000-0002-5161-9722}} % 2236
  \author{M.~Khan\,\orcidlink{0000-0002-2168-0872}} % 15644
  \author{C.~Kiesling\,\orcidlink{0000-0002-2209-535X}} % 2168
% \author{C.~Kim\,\orcidlink{0009-0000-9835-9625}} % 20503
% \author{C.-H.~Kim\,\orcidlink{0000-0002-5743-7698}} % 2358
  \author{D.~Y.~Kim\,\orcidlink{0000-0001-8125-9070}} % 2315
  \author{J.-Y.~Kim\,\orcidlink{0000-0001-7593-843X}} % 20223
  \author{K.-H.~Kim\,\orcidlink{0000-0002-4659-1112}} % 2118
% \author{S.~K.~Kim\,\orcidlink{-}} % 3823
% \author{Y.~J.~Kim\,\orcidlink{0000-0001-9511-9634}} % 2403
% \author{Y.-K.~Kim\,\orcidlink{0000-0002-9695-8103}} % 2379
% \author{H.~Kindo\,\orcidlink{0000-0002-6756-3591}} % 2195
  \author{K.~Kinoshita\,\orcidlink{0000-0001-7175-4182}} % 2318
  \author{P.~Kody\v{s}\,\orcidlink{0000-0002-8644-2349}} % 2407
  \author{T.~Koga\,\orcidlink{0000-0002-1644-2001}} % 6963
  \author{S.~Kohani\,\orcidlink{0000-0003-3869-6552}} % 9143
  \author{K.~Kojima\,\orcidlink{0000-0002-3638-0266}} % 6363
% \author{T.~Konno\,\orcidlink{0000-0003-2487-8080}} % 2490
% \author{H.~Korandla\,\orcidlink{0000-0003-0516-7793}} % 18783
  \author{A.~Korobov\,\orcidlink{0000-0001-5959-8172}} % 4185
  \author{S.~Korpar\,\orcidlink{0000-0003-0971-0968}} % 2475
% \author{E.~Kou\,\orcidlink{0000-0002-8650-6699}} % 3765
  \author{E.~Kovalenko\,\orcidlink{0000-0001-8084-1931}} % 3884
  \author{R.~Kowalewski\,\orcidlink{0000-0002-7314-0990}} % 2293
% \author{T.~M.~G.~Kraetzschmar\,\orcidlink{0000-0001-8395-2928}} % 7543
  \author{P.~Kri\v{z}an\,\orcidlink{0000-0002-4967-7675}} % 2474
% \author{R.~Kroeger\,\orcidlink{-}} % 2242
  \author{P.~Krokovny\,\orcidlink{0000-0002-1236-4667}} % 2575
% \author{W.~Kuehn\,\orcidlink{0000-0001-6018-9878}} % 2534
% \author{T.~Kuhr\,\orcidlink{0000-0001-6251-8049}} % 2486
% \author{Y.~Kulii\,\orcidlink{0000-0001-6217-5162}} % 9823
% \author{D.~Kumar\,\orcidlink{0000-0001-6585-7767}} % 7223
% \author{J.~Kumar\,\orcidlink{0000-0002-8465-433X}} % 6464
% \author{M.~Kumar\,\orcidlink{0000-0002-6627-9708}} % 2744
% \author{R.~Kumar\,\orcidlink{0000-0002-6277-2626}} % 2189
  \author{K.~Kumara\,\orcidlink{0000-0003-1572-5365}} % 2257
% \author{T.~Kumita\,\orcidlink{0000-0001-7572-4538}} % 4083
  \author{T.~Kunigo\,\orcidlink{0000-0001-9613-2849}} % 10104
% \author{A.~Kusudo\,\orcidlink{0000-0002-2662-9734}} % 14623
  \author{A.~Kuzmin\,\orcidlink{0000-0002-7011-5044}} % 2520
% \author{P.~Kvasni\v{c}ka\,\orcidlink{0000-0001-6281-0648}} % 2184
  \author{Y.-J.~Kwon\,\orcidlink{0000-0001-9448-5691}} % 2231
% \author{S.~Lacaprara\,\orcidlink{0000-0002-0551-7696}} % 2447
% \author{Y.-T.~Lai\,\orcidlink{0000-0001-9553-3421}} % 2066
  \author{K.~Lalwani\,\orcidlink{0000-0002-7294-396X}} % 2142
  \author{T.~Lam\,\orcidlink{0000-0001-9128-6806}} % 2729
% \author{L.~Lanceri\,\orcidlink{0000-0001-8220-3095}} % 2540
  \author{J.~S.~Lange\,\orcidlink{0000-0003-0234-0474}} % 2277
  \author{T.~S.~Lau\,\orcidlink{0000-0001-7110-7823}} % 19803
  \author{M.~Laurenza\,\orcidlink{0000-0002-7400-6013}} % 10223
% \author{K.~Lautenbach\,\orcidlink{0000-0003-3762-694X}} % 2102
% \author{P.~J.~Laycock\,\orcidlink{0000-0002-8572-5339}} % 7683
  \author{R.~Leboucher\,\orcidlink{0000-0003-3097-6613}} % 14083
  \author{F.~R.~Le~Diberder\,\orcidlink{0000-0002-9073-5689}} % 3267
  \author{M.~J.~Lee\,\orcidlink{0000-0003-4528-4601}} % 21803
% \author{P.~Leitl\,\orcidlink{0000-0002-1336-9558}} % 2414
  \author{C.~Lemettais\,\orcidlink{0009-0008-5394-5100}} % 22704
  \author{P.~Leo\,\orcidlink{0000-0003-3833-2900}} % 19823
% \author{D.~Levit\,\orcidlink{0000-0001-5789-6205}} % 2507
% \author{P.~M.~Lewis\,\orcidlink{0000-0002-5991-622X}} % 2582
% \author{C.~Li\,\orcidlink{0000-0002-3240-4523}} % 2325
  \author{H.-J.~Li\,\orcidlink{0000-0001-9275-4739}} % 4943
  \author{L.~K.~Li\,\orcidlink{0000-0002-7366-1307}} % 3263
  \author{Q.~M.~Li\,\orcidlink{0009-0004-9425-2678}} % 22943
% \author{S.~X.~Li\,\orcidlink{0000-0003-4669-1495}} % 2377
  \author{W.~Z.~Li\,\orcidlink{0009-0002-8040-2546}} % 19703
  \author{Y.~Li\,\orcidlink{0000-0002-4413-6247}} % 8083
  \author{Y.~B.~Li\,\orcidlink{0000-0002-9909-2851}} % 2573
  \author{Y.~P.~Liao\,\orcidlink{0009-0000-1981-0044}} % 24303
  \author{J.~Libby\,\orcidlink{0000-0002-1219-3247}} % 2262
  \author{J.~Lin\,\orcidlink{0000-0002-3653-2899}} % 2401
  \author{S.~Lin\,\orcidlink{0000-0001-5922-9561}} % 17223
% \author{Z.~Liptak\,\orcidlink{0000-0002-6491-8131}} % 3565
  \author{V.~Lisovskyi\,\orcidlink{0000-0003-4451-214X}} % 26584
% \author{A.~Little\,\orcidlink{0009-0008-4974-3661}} % 23803
  \author{M.~H.~Liu\,\orcidlink{0000-0002-9376-1487}} % 15244
  \author{Q.~Y.~Liu\,\orcidlink{0000-0002-7684-0415}} % 7045
  \author{Y.~Liu\,\orcidlink{0000-0002-8374-3947}} % 16223
  \author{Z.~Liu\,\orcidlink{0000-0002-0290-3022}} % 11303
% \author{Z.~A.~Liu\,\orcidlink{0000-0002-2896-1386}} % 3283
  \author{D.~Liventsev\,\orcidlink{0000-0003-3416-0056}} % 2578
  \author{S.~Longo\,\orcidlink{0000-0002-8124-8969}} % 2396
% \author{G.~Lopez-Castro\,\orcidlink{-}} % 4245
% \author{A.~Lozar\,\orcidlink{0000-0002-0569-6882}} % 12423
% \author{T.~Lueck\,\orcidlink{0000-0003-3915-2506}} % 2406
% \author{T.~Luo\,\orcidlink{0000-0001-5139-5784}} % 3268
  \author{C.~Lyu\,\orcidlink{0000-0002-2275-0473}} % 12484
  \author{Y.~Ma\,\orcidlink{0000-0001-8412-8308}} % 16883
  \author{C.~Madaan\,\orcidlink{0009-0004-1205-5700}} % 25483
% \author{A.~Maeda\,\orcidlink{0009-0009-8839-7148}} % 14664
  \author{M.~Maggiora\,\orcidlink{0000-0003-4143-9127}} % 5343
  \author{S.~P.~Maharana\,\orcidlink{0000-0002-1746-4683}} % 19083
% \author{T.~Mahood\,\orcidlink{0009-0004-3017-6661}} % 26003
  \author{R.~Maiti\,\orcidlink{0000-0001-5534-7149}} % 12043
% \author{S.~Maity\,\orcidlink{0000-0003-3076-9243}} % 2985
  \author{G.~Mancinelli\,\orcidlink{0000-0003-1144-3678}} % 20743
  \author{R.~Manfredi\,\orcidlink{0000-0002-8552-6276}} % 10303
  \author{E.~Manoni\,\orcidlink{0000-0002-9826-7947}} % 2305
% \author{A.~C.~Manthei\,\orcidlink{0000-0002-6900-5729}} % 15023
  \author{M.~Mantovano\,\orcidlink{0000-0002-5979-5050}} % 19783
  \author{D.~Marcantonio\,\orcidlink{0000-0002-1315-8646}} % 11163
  \author{S.~Marcello\,\orcidlink{0000-0003-4144-863X}} % 4223
  \author{C.~Marinas\,\orcidlink{0000-0003-1903-3251}} % 2133
  \author{C.~Martellini\,\orcidlink{0000-0002-7189-8343}} % 16983
  \author{A.~Martens\,\orcidlink{0000-0003-1544-4053}} % 13823
% \author{A.~Martini\,\orcidlink{0000-0003-1161-4983}} % 2336
  \author{T.~Martinov\,\orcidlink{0000-0001-7846-1913}} % 19463
  \author{L.~Massaccesi\,\orcidlink{0000-0003-1762-4699}} % 16323
  \author{M.~Masuda\,\orcidlink{0000-0002-7109-5583}} % 2238
% \author{T.~Matsuda\,\orcidlink{0000-0003-4673-570X}} % 5543
% \author{K.~Matsuoka\,\orcidlink{0000-0003-1706-9365}} % 2316
% \author{D.~Matvienko\,\orcidlink{0000-0002-2698-5448}} % 2351
  \author{S.~K.~Maurya\,\orcidlink{0000-0002-7764-5777}} % 9763
  \author{M.~Maushart\,\orcidlink{0009-0004-1020-7299}} % 21203
% \author{F.~Mawas\,\orcidlink{0000-0002-7176-4732}} % 20943
  \author{J.~A.~McKenna\,\orcidlink{0000-0001-9871-9002}} % 2392
% \author{F.~Meggendorfer\,\orcidlink{0000-0002-1466-7207}} % 7103
% \author{R.~Mehta\,\orcidlink{0000-0001-8670-3409}} % 15203
  \author{F.~Meier\,\orcidlink{0000-0002-6088-0412}} % 3103
  \author{D.~Meleshko\,\orcidlink{0000-0002-0872-4623}} % 11523
  \author{M.~Merola\,\orcidlink{0000-0002-7082-8108}} % 2456
% \author{F.~Metzner\,\orcidlink{0000-0002-0128-264X}} % 2296
% \author{M.~Milesi\,\orcidlink{0000-0002-8805-1886}} % 5443
  \author{C.~Miller\,\orcidlink{0000-0003-2631-1790}} % 2273
  \author{M.~Mirra\,\orcidlink{0000-0002-1190-2961}} % 14744
  \author{S.~Mitra\,\orcidlink{0000-0002-1118-6344}} % 19944
  \author{K.~Miyabayashi\,\orcidlink{0000-0003-4352-734X}} % 2327
% \author{H.~Miyake\,\orcidlink{0000-0002-7079-8236}} % 2452
  \author{R.~Mizuk\,\orcidlink{0000-0002-2209-6969}} % 2483
  \author{G.~B.~Mohanty\,\orcidlink{0000-0001-6850-7666}} % 2278
% \author{S.~Mondal\,\orcidlink{0000-0002-3054-8400}} % 19743
  \author{S.~Moneta\,\orcidlink{0000-0003-2184-7510}} % 13303
% \author{H.~Moon\,\orcidlink{0000-0001-5213-6477}} % 2304
% \author{A.~L.~Moreira~de~Carvalho\,\orcidlink{0000-0002-1986-5720}} % 26403
  \author{H.-G.~Moser\,\orcidlink{0000-0003-3579-9951}} % 2120
% \author{M.~Mrvar\,\orcidlink{0000-0001-6388-3005}} % 2527
% \author{Th.~Muller\,\orcidlink{0000-0003-4337-0098}} % 2165
% \author{R.~Mussa\,\orcidlink{0000-0002-0294-9071}} % 2372
% \author{I.~Nakamura\,\orcidlink{0000-0002-7640-5456}} % 3463
% \author{K.~R.~Nakamura\,\orcidlink{0000-0001-7012-7355}} % 2417
% \author{E.~Nakano\,\orcidlink{0000-0003-2282-5217}} % 2554
% \author{T.~Nakano\,\orcidlink{0000-0003-3157-5328}} % 2983
  \author{M.~Nakao\,\orcidlink{0000-0001-8424-7075}} % 2498
% \author{H.~Nakayama\,\orcidlink{0000-0002-2030-9967}} % 2232
  \author{H.~Nakazawa\,\orcidlink{0000-0003-1684-6628}} % 2335
  \author{Y.~Nakazawa\,\orcidlink{0000-0002-6271-5808}} % 17383
% \author{A.~Narimani~Charan\,\orcidlink{0000-0002-5975-550X}} % 10143
  \author{M.~Naruki\,\orcidlink{0000-0003-1773-2999}} % 4583
  \author{Z.~Natkaniec\,\orcidlink{0000-0003-0486-9291}} % 3923
  \author{A.~Natochii\,\orcidlink{0000-0002-1076-814X}} % 12063
% \author{L.~Nayak\,\orcidlink{0000-0002-7739-914X}} % 9464
  \author{M.~Nayak\,\orcidlink{0000-0002-2572-4692}} % 2371
% \author{G.~Nazaryan\,\orcidlink{0000-0002-9434-6197}} % 9523
  \author{M.~Neu\,\orcidlink{0000-0002-4564-8009}} % 23304
% \author{C.~Niebuhr\,\orcidlink{0000-0002-4375-9741}} % 2477
% \author{M.~Niiyama\,\orcidlink{0000-0003-1746-586X}} % 2063
% \author{J.~Ninkovic\,\orcidlink{0000-0003-1523-3635}} % 2386
% \author{N.~K.~Nisar\,\orcidlink{0000-0001-9562-1253}} % 2522
  \author{S.~Nishida\,\orcidlink{0000-0001-6373-2346}} % 2571
% \author{K.~Nishimura\,\orcidlink{0000-0001-8818-8922}} % 3063
% \author{A.~Novosel\,\orcidlink{0000-0002-7308-8950}} % 15523
  \author{S.~Ogawa\,\orcidlink{0000-0002-7310-5079}} % 6263
  \author{R.~Okubo\,\orcidlink{0009-0009-0912-0678}} % 10743
% \author{S.~L.~Olsen\,\orcidlink{0000-0002-6388-9885}} % 4563
  \author{H.~Ono\,\orcidlink{0000-0003-4486-0064}} % 2160
% \author{Y.~Onuki\,\orcidlink{0000-0002-1646-6847}} % 2331
% \author{P.~Oskin\,\orcidlink{0000-0002-7524-0936}} % 9623
% \author{F.~Otani\,\orcidlink{0000-0001-6016-219X}} % 16244
  \author{E.~R.~Oxford\,\orcidlink{0000-0002-0813-4578}} % 6943
% \author{H.~Ozaki\,\orcidlink{0000-0001-6901-1881}} % 2984
% \author{P.~Pakhlov\,\orcidlink{0000-0001-7426-4824}} % 2221
  \author{G.~Pakhlova\,\orcidlink{0000-0001-7518-3022}} % 2188
% \author{A.~Panta\,\orcidlink{0000-0001-6385-7712}} % 7943
% \author{E.~Paoloni\,\orcidlink{0000-0001-5969-8712}} % 2488
  \author{S.~Pardi\,\orcidlink{0000-0001-7994-0537}} % 2532
  \author{K.~Parham\,\orcidlink{0000-0001-9556-2433}} % 10684
  \author{H.~Park\,\orcidlink{0000-0001-6087-2052}} % 2284
  \author{J.~Park\,\orcidlink{0000-0001-6520-0028}} % 18203
  \author{K.~Park\,\orcidlink{0000-0003-0567-3493}} % 12243
  \author{S.-H.~Park\,\orcidlink{0000-0001-6019-6218}} % 2509
% \author{B.~Paschen\,\orcidlink{0000-0003-1546-4548}} % 2159
  \author{A.~Passeri\,\orcidlink{0000-0003-4864-3411}} % 2116
  \author{S.~Patra\,\orcidlink{0000-0002-4114-1091}} % 3123
% \author{S.~Paul\,\orcidlink{0000-0002-8813-0437}} % 2131
% \author{T.~K.~Pedlar\,\orcidlink{0000-0001-9839-7373}} % 2421
% \author{I.~Peruzzi\,\orcidlink{0000-0001-6729-8436}} % 2253
% \author{R.~Peschke\,\orcidlink{0000-0002-2529-8515}} % 7123
  \author{R.~Pestotnik\,\orcidlink{0000-0003-1804-9470}} % 2476
% \author{F.~Pham\,\orcidlink{0000-0003-0608-2302}} % 2963
% \author{M.~Piccolo\,\orcidlink{0000-0001-9750-0551}} % 2147
  \author{L.~E.~Piilonen\,\orcidlink{0000-0001-6836-0748}} % 2346
  \author{P.~L.~M.~Podesta-Lerma\,\orcidlink{0000-0002-8152-9605}} % 2266
  \author{T.~Podobnik\,\orcidlink{0000-0002-6131-819X}} % 11223
% \author{S.~Pokharel\,\orcidlink{0000-0002-3367-738X}} % 12283
% \author{V.~Popov\,\orcidlink{0000-0003-0208-2583}} % 2096
  \author{A.~Prakash\,\orcidlink{0000-0002-6462-8142}} % 21663
  \author{C.~Praz\,\orcidlink{0000-0002-6154-885X}} % 2726
  \author{S.~Prell\,\orcidlink{0000-0002-0195-8005}} % 12743
  \author{E.~Prencipe\,\orcidlink{0000-0002-9465-2493}} % 2219
  \author{M.~T.~Prim\,\orcidlink{0000-0002-1407-7450}} % 2501
  \author{S.~Privalov\,\orcidlink{0009-0004-1681-3919}} % 12503
% \author{I.~Prudiiev\,\orcidlink{0000-0002-0819-284X}} % 19383
% \author{M.~V.~Purohit\,\orcidlink{0000-0002-8381-8689}} % 2196
  \author{H.~Purwar\,\orcidlink{0000-0002-3876-7069}} % 12363
% \author{N.~Rad\,\orcidlink{0000-0002-5204-0851}} % 11683
  \author{P.~Rados\,\orcidlink{0000-0003-0690-8100}} % 7383
  \author{G.~Raeuber\,\orcidlink{0000-0003-2948-5155}} % 18143
  \author{S.~Raiz\,\orcidlink{0000-0001-7010-8066}} % 13003
  \author{V.~Raj\,\orcidlink{0009-0003-2433-8065}} % 24983
% \author{N.~Rauls\,\orcidlink{0000-0002-6583-4888}} % 11603
  \author{K.~Ravindran\,\orcidlink{0000-0002-5584-2614}} % 22503
  \author{J.~U.~Rehman\,\orcidlink{0000-0002-2673-1982}} % 19623
  \author{M.~Reif\,\orcidlink{0000-0002-0706-0247}} % 8043
  \author{S.~Reiter\,\orcidlink{0000-0002-6542-9954}} % 2248
  \author{M.~Remnev\,\orcidlink{0000-0001-6975-1724}} % 2785
  \author{L.~Reuter\,\orcidlink{0000-0002-5930-6237}} % 16403
  \author{D.~Ricalde~Herrmann\,\orcidlink{0000-0001-9772-9989}} % 9263
  \author{I.~Ripp-Baudot\,\orcidlink{0000-0002-1897-8272}} % 2469
% \author{M.~Ritzert\,\orcidlink{0000-0003-2928-7044}} % 2526
  \author{G.~Rizzo\,\orcidlink{0000-0003-1788-2866}} % 2579
% \author{L.~B.~Rizzuto\,\orcidlink{0000-0001-6621-6646}} % 3746
% \author{S.~H.~Robertson\,\orcidlink{0000-0003-4096-8393}} % 2471
% \author{P.~Rocchetti\,\orcidlink{0000-0002-2839-3489}} % 13763
% \author{D.~Rodr\'{i}guez~P\'{e}rez\,\orcidlink{0000-0001-8505-649X}} % 2176
% \author{M.~Roehrken\,\orcidlink{0000-0003-0654-2866}} % 11883
  \author{J.~M.~Roney\,\orcidlink{0000-0001-7802-4617}} % 2244
% \author{C.~Rosenfeld\,\orcidlink{0000-0003-3857-1223}} % 2082
  \author{A.~Rostomyan\,\orcidlink{0000-0003-1839-8152}} % 2481
  \author{N.~Rout\,\orcidlink{0000-0002-4310-3638}} % 2965
% \author{M.~Rozanska\,\orcidlink{0000-0003-2651-5021}} % 2205
% \author{G.~Russo\,\orcidlink{0000-0001-5823-4393}} % 2388
% \author{D.~Sahoo\,\orcidlink{0000-0002-5600-9413}} % 2110
% \author{Y.~Sakai\,\orcidlink{0000-0001-9163-3409}} % 2175
  \author{L.~Salutari\,\orcidlink{0009-0001-2822-6939}} % 17423
% \author{G.~Sanchez\,\orcidlink{0000-0003-4824-9983}} % 2943
  \author{D.~A.~Sanders\,\orcidlink{0000-0002-4902-966X}} % 2458
  \author{S.~Sandilya\,\orcidlink{0000-0002-4199-4369}} % 2286
% \author{A.~Sangal\,\orcidlink{0000-0001-5853-349X}} % 2384
  \author{L.~Santelj\,\orcidlink{0000-0003-3904-2956}} % 2185
% \author{C.~Santos\,\orcidlink{0009-0005-2430-1670}} % 23743
% \author{Y.~Sato\,\orcidlink{0000-0003-3751-2803}} % 5243
  \author{V.~Savinov\,\orcidlink{0000-0002-9184-2830}} % 2292
  \author{B.~Scavino\,\orcidlink{0000-0003-1771-9161}} % 2518
  \author{C.~Schmitt\,\orcidlink{0000-0002-3787-687X}} % 15063
  \author{J.~Schmitz\,\orcidlink{0000-0001-8274-8124}} % 12863
  \author{S.~Schneider\,\orcidlink{0009-0002-5899-0353}} % 16803
  \author{M.~Schnepf\,\orcidlink{0000-0003-0623-0184}} % 15683
% \author{K.~Schoenning\,\orcidlink{0000-0002-3490-9584}} % 22023
% \author{J.~Schueler\,\orcidlink{0000-0002-2722-6953}} % 2824
  \author{C.~Schwanda\,\orcidlink{0000-0003-4844-5028}} % 2108
  \author{A.~J.~Schwartz\,\orcidlink{0000-0002-7310-1983}} % 2162
% \author{B.~Schwenker\,\orcidlink{0000-0002-7120-3732}} % 2405
% \author{M.~Schwickardi\,\orcidlink{0000-0003-2033-6700}} % 14743
  \author{Y.~Seino\,\orcidlink{0000-0002-8378-4255}} % 2517
  \author{A.~Selce\,\orcidlink{0000-0001-8228-9781}} % 9043
  \author{K.~Senyo\,\orcidlink{0000-0002-1615-9118}} % 2987
  \author{J.~Serrano\,\orcidlink{0000-0003-2489-7812}} % 12124
  \author{M.~E.~Sevior\,\orcidlink{0000-0002-4824-101X}} % 2328
  \author{C.~Sfienti\,\orcidlink{0000-0002-5921-8819}} % 2214
  \author{W.~Shan\,\orcidlink{0000-0003-2811-2218}} % 11943
% \author{C.~Sharma\,\orcidlink{0000-0002-1312-0429}} % 11584
% \author{G.~Sharma\,\orcidlink{0000-0002-5620-5334}} % 18423
% \author{V.~Shebalin\,\orcidlink{0000-0003-1012-0957}} % 2339
% \author{C.~P.~Shen\,\orcidlink{0000-0002-9012-4618}} % 2464
  \author{X.~D.~Shi\,\orcidlink{0000-0002-7006-6107}} % 18843
% \author{H.~Shibuya\,\orcidlink{0000-0002-0197-6270}} % 2234
  \author{T.~Shillington\,\orcidlink{0000-0003-3862-4380}} % 7983
% \author{T.~Shimasaki\,\orcidlink{0000-0003-3291-9532}} % 16263
% \author{M.~Shimomura\,\orcidlink{0000-0001-9598-779X}} % 2112
  \author{J.-G.~Shiu\,\orcidlink{0000-0002-8478-5639}} % 2412
  \author{D.~Shtol\,\orcidlink{0000-0002-0622-6065}} % 9223
  \author{B.~Shwartz\,\orcidlink{0000-0002-1456-1496}} % 2122
  \author{A.~Sibidanov\,\orcidlink{0000-0001-8805-4895}} % 2419
  \author{F.~Simon\,\orcidlink{0000-0002-5978-0289}} % 2164
% \author{J.~B.~Singh\,\orcidlink{0000-0001-9029-2462}} % 2903
  \author{J.~Skorupa\,\orcidlink{0000-0002-8566-621X}} % 12523
% \author{K.~Smith\,\orcidlink{0000-0003-0446-9474}} % 2243
  \author{R.~J.~Sobie\,\orcidlink{0000-0001-7430-7599}} % 2472
  \author{M.~Sobotzik\,\orcidlink{0000-0002-1773-5455}} % 8604
  \author{A.~Soffer\,\orcidlink{0000-0002-0749-2146}} % 2217
  \author{A.~Sokolov\,\orcidlink{0000-0002-9420-0091}} % 2521
% \author{Y.~Soloviev\,\orcidlink{0000-0003-1136-2827}} % 2479
  \author{E.~Solovieva\,\orcidlink{0000-0002-5735-4059}} % 2398
% \author{W.~Song\,\orcidlink{0000-0003-1376-2293}} % 22863
  \author{S.~Spataro\,\orcidlink{0000-0001-9601-405X}} % 2117
  \author{B.~Spruck\,\orcidlink{0000-0002-3060-2729}} % 2493
% \author{S.~Stani\v{c}\,\orcidlink{0000-0003-3344-8381}} % 3383
  \author{M.~Stari\v{c}\,\orcidlink{0000-0001-8751-5944}} % 2326
  \author{P.~Stavroulakis\,\orcidlink{0000-0001-9914-7261}} % 20643
  \author{S.~Stefkova\,\orcidlink{0000-0003-2628-530X}} % 8783
% \author{L.~Stoetzer\,\orcidlink{0009-0003-2245-1603}} % 19283
% \author{Z.~S.~Stottler\,\orcidlink{0000-0002-1898-5333}} % 2267
  \author{R.~Stroili\,\orcidlink{0000-0002-3453-142X}} % 2465
% \author{J.~Strube\,\orcidlink{0000-0001-7470-9301}} % 2451
% \author{J.~Su\,\orcidlink{0009-0001-1644-8198}} % 16623
  \author{Y.~Sue\,\orcidlink{0000-0003-2430-8707}} % 2085
% \author{R.~Sugiura\,\orcidlink{0000-0002-6044-5445}} % 4644
  \author{M.~Sumihama\,\orcidlink{0000-0002-8954-0585}} % 4243
% \author{K.~Sumisawa\,\orcidlink{0000-0001-7003-7210}} % 2583
% \author{W.~Sutcliffe\,\orcidlink{0000-0002-9795-3582}} % 3784
  \author{N.~Suwonjandee\,\orcidlink{0009-0000-2819-5020}} % 14063
  \author{H.~Svidras\,\orcidlink{0000-0003-4198-2517}} % 11783
% \author{M.~Takahashi\,\orcidlink{0000-0003-1171-5960}} % 2467
  \author{M.~Takizawa\,\orcidlink{0000-0001-8225-3973}} % 2437
% \author{U.~Tamponi\,\orcidlink{0000-0001-6651-0706}} % 2366
% \author{S.~Tanaka\,\orcidlink{0000-0002-6029-6216}} % 2530
  \author{K.~Tanida\,\orcidlink{0000-0002-8255-3746}} % 3803
% \author{H.~Tanigawa\,\orcidlink{0000-0003-3681-9985}} % 2237
% \author{N.~Taniguchi\,\orcidlink{0000-0002-1462-0564}} % 2285
  \author{F.~Tenchini\,\orcidlink{0000-0003-3469-9377}} % 2546
  \author{F.~Testa\,\orcidlink{0009-0004-5075-8247}} % 14844
% \author{A.~Thaller\,\orcidlink{0000-0003-4171-6219}} % 16044
  \author{O.~Tittel\,\orcidlink{0000-0001-9128-6240}} % 8663
  \author{R.~Tiwary\,\orcidlink{0000-0002-5887-1883}} % 10403
% \author{D.~Tonelli\,\orcidlink{0000-0002-1494-7882}} % 4564
  \author{E.~Torassa\,\orcidlink{0000-0003-2321-0599}} % 2556
% \author{N.~Toutounji\,\orcidlink{0000-0002-1937-6732}} % 2263
  \author{K.~Trabelsi\,\orcidlink{0000-0001-6567-3036}} % 2369
  \author{F.~F.~Trantou\,\orcidlink{0000-0003-0517-9129}} % 23643
  \author{I.~Tsaklidis\,\orcidlink{0000-0003-3584-4484}} % 13443
% \author{T.~Tsuboyama\,\orcidlink{0000-0002-4575-1997}} % 2361
% \author{N.~Tsuzuki\,\orcidlink{0000-0003-1141-1908}} % 2352
  \author{M.~Uchida\,\orcidlink{0000-0003-4904-6168}} % 2370
  \author{I.~Ueda\,\orcidlink{0000-0002-6833-4344}} % 2519
% \author{S.~Uehara\,\orcidlink{0000-0001-7377-5016}} % 2586
% \author{Y.~Uematsu\,\orcidlink{0000-0002-0296-4028}} % 5883
% \author{E.~Uenlue\,\orcidlink{0009-0000-3417-6790}} % 22283
  \author{T.~Uglov\,\orcidlink{0000-0002-4944-1830}} % 2252
  \author{K.~Unger\,\orcidlink{0000-0001-7378-6671}} % 9463
  \author{Y.~Unno\,\orcidlink{0000-0003-3355-765X}} % 2420
  \author{K.~Uno\,\orcidlink{0000-0002-2209-8198}} % 14963
  \author{S.~Uno\,\orcidlink{0000-0002-3401-0480}} % 2149
% \author{P.~Urquijo\,\orcidlink{0000-0002-0887-7953}} % 2302
  \author{Y.~Ushiroda\,\orcidlink{0000-0003-3174-403X}} % 2317
% \author{Y.~V.~Usov\,\orcidlink{0000-0003-3144-2920}} % 5003
% \author{S.~E.~Vahsen\,\orcidlink{0000-0003-1685-9824}} % 2251
  \author{R.~van~Tonder\,\orcidlink{0000-0002-7448-4816}} % 2706
  \author{K.~E.~Varvell\,\orcidlink{0000-0003-1017-1295}} % 2545
  \author{M.~Veronesi\,\orcidlink{0000-0002-1916-3884}} % 20723
  \author{A.~Vinokurova\,\orcidlink{0000-0003-4220-8056}} % 2289
  \author{V.~S.~Vismaya\,\orcidlink{0000-0002-1606-5349}} % 16063
  \author{L.~Vitale\,\orcidlink{0000-0003-3354-2300}} % 2415
% \author{V.~Vobbilisetti\,\orcidlink{0000-0002-4399-5082}} % 7364
  \author{R.~Volpe\,\orcidlink{0000-0003-1782-2978}} % 20183
  \author{A.~Vossen\,\orcidlink{0000-0003-0983-4936}} % 2249
% \author{B.~Wach\,\orcidlink{0000-0003-3533-7669}} % 8203
% \author{E.~Waheed\,\orcidlink{0000-0001-7774-0363}} % 2226
% \author{M.~Wakai\,\orcidlink{0000-0003-2818-3155}} % 3583
% \author{H.~M.~Wakeling\,\orcidlink{0000-0003-4606-7895}} % 3664
  \author{S.~Wallner\,\orcidlink{0000-0002-9105-1625}} % 20363
% \author{W.~Wan~Abdullah\,\orcidlink{0000-0001-5798-9145}} % 2280
% \author{B.~Wang\,\orcidlink{0000-0001-6136-6952}} % 2569
% \author{E.~Wang\,\orcidlink{0000-0001-6391-5118}} % 10983
% \author{L.~Wang\,\orcidlink{0000-0003-2464-6239}} % 22443
  \author{M.-Z.~Wang\,\orcidlink{0000-0002-0979-8341}} % 2074
% \author{X.~L.~Wang\,\orcidlink{0000-0001-5805-1255}} % 2076
% \author{Z.~Wang\,\orcidlink{0000-0002-3536-4950}} % 15743
  \author{A.~Warburton\,\orcidlink{0000-0002-2298-7315}} % 2347
  \author{M.~Watanabe\,\orcidlink{0000-0001-6917-6694}} % 2309
  \author{S.~Watanuki\,\orcidlink{0000-0002-5241-6628}} % 6843
% \author{M.~Welsch\,\orcidlink{0000-0002-3026-1872}} % 7023
% \author{O.~Werbycka\,\orcidlink{0000-0002-0614-8773}} % 6123
  \author{C.~Wessel\,\orcidlink{0000-0003-0959-4784}} % 2100
% \author{J.~Wiechczynski\,\orcidlink{0000-0002-3151-6072}} % 2604
  \author{E.~Won\,\orcidlink{0000-0002-4245-7442}} % 2410
% \author{Y.~Xie\,\orcidlink{0000-0002-0170-2798}} % 20383
% \author{X.~P.~Xu\,\orcidlink{0000-0001-5096-1182}} % 4923
% \author{Z.~Xu\,\orcidlink{0009-0005-1048-4744}} % 27103
  \author{B.~D.~Yabsley\,\orcidlink{0000-0002-2680-0474}} % 3645
  \author{S.~Yamada\,\orcidlink{0000-0002-8858-9336}} % 2492
  \author{W.~Yan\,\orcidlink{0000-0003-0713-0871}} % 2094
% \author{W.~C.~Yan\,\orcidlink{0000-0001-6721-9435}} % 2183
  \author{S.~B.~Yang\,\orcidlink{0000-0002-9543-7971}} % 2374
  \author{J.~Yelton\,\orcidlink{0000-0001-8840-3346}} % 2067
  \author{J.~H.~Yin\,\orcidlink{0000-0002-1479-9349}} % 2365
% \author{Y.~M.~Yook\,\orcidlink{0000-0002-4912-048X}} % 2453
  \author{K.~Yoshihara\,\orcidlink{0000-0002-3656-2326}} % 12663
% \author{B.~Yu\,\orcidlink{0000-0002-2437-7289}} % 15563
% \author{C.~Z.~Yuan\,\orcidlink{0000-0002-1652-6686}} % 2088
  \author{J.~Yuan\,\orcidlink{0009-0005-0799-1630}} % 23423
  \author{Y.~Yusa\,\orcidlink{0000-0002-4001-9748}} % 2357
  \author{L.~Zani\,\orcidlink{0000-0003-4957-805X}} % 2529
% \author{F.~Zeng\,\orcidlink{0009-0003-6474-3508}} % 22043
  \author{M.~Zeyrek\,\orcidlink{0000-0002-9270-7403}} % 4023
  \author{B.~Zhang\,\orcidlink{0000-0002-5065-8762}} % 11663
% \author{J.~Z.~Zhang\,\orcidlink{0000-0001-6535-0659}} % 2349
% \author{Y.~Zhang\,\orcidlink{0000-0003-2961-2820}} % 3303
% \author{Z.~Zhang\,\orcidlink{0000-0001-6140-2044}} % 5363
% \author{J.~Zhao\,\orcidlink{-}} % 3343
  \author{V.~Zhilich\,\orcidlink{0000-0002-0907-5565}} % 4703
  \author{J.~S.~Zhou\,\orcidlink{0000-0002-6413-4687}} % 12463
  \author{Q.~D.~Zhou\,\orcidlink{0000-0001-5968-6359}} % 7323
% \author{X.~Y.~Zhou\,\orcidlink{0000-0002-0299-4657}} % 2380
  \author{L.~Zhu\,\orcidlink{0009-0007-1127-5818}} % 25143
% \author{V.~I.~Zhukova\,\orcidlink{0000-0002-8253-641X}} % 2387
% \author{V.~Zhulanov\,\orcidlink{0000-0002-0306-9199}} % 4983
  \author{R.~\v{Z}leb\v{c}\'{i}k\,\orcidlink{0000-0003-1644-8523}} % 13403
% \author{S.~Zou\,\orcidlink{0000-0003-3377-7222}} % 19363
\collaboration{The Belle II Collaboration}

